Efficient and Interpretable Bandit Algorithms

Motivated by the importance of explainability in modern machine learning, we design bandit algorithms that are efficient and interpretable. A bandit algorithm is interpretable if it explores with the objective of reducing uncertainty in the unknown model parameter. To quantify the interpretability, we introduce a novel metric of model error, which compares the rate reduction of the mean reward estimates to their actual means among all the plausible actions. We propose CODE, a bandit algorithm based on a Constrained Optimal DEsign, that is interpretable and maximally reduces the uncertainty. The key idea in CODE is to explore among all plausible actions, determined by a statistical constraint, to achieve interpretability. We implement CODE efficiently in both multi-armed and linear bandits and derive near-optimal regret bounds by leveraging the optimality criteria of the approximate optimal design. CODE can be also viewed as removing phases in conventional phased elimination, which makes it more practical and general. We demonstrate the advantage of CODE by numerical experiments on both synthetic and real-world problems. CODE outperforms other state-of-the-art interpretable designs while matching the performance of popular but uninterpretable designs, such as upper confidence bound algorithms.

==> backup.tex <==
{\color{red} Start of paper outline}

\textbf{Section 1: Introduction}

\textbf{Section 2: Background}

* A lot of good work has been done on regret minimization. But many challenges remain:

o Exploration is hard to control. This is why practitioners prefer the $\varepsilon$-greedy policy. Conservative bandits are always an option. This takes care of only one particular constraint, that the exploration policy is close to the production policy.
\todoz{I would suggest we do not include this as it is a bit of distraction. Explainability and the easiness of including side constraints seem enough and they are directly addressed. Maybe I am wrong, but why do we think our approach can control exploration more easily?}

o Side constraints are hard to incorporate. Motivate the need. Promotions in marketing. Fairness. A lot of work on side constraints recently.

o TS and UCB are hard to explain. TS can be explained by sampling many times from the posterior and computing the empirical distribution over the pulled arms. The $\varepsilon$-greedy policy is easy to explain.

* I like doing related work at the end of the paper. In this case though, it seems natural to do it at the beginning.

\textbf{Section 3: Setting}

* We have a linear bandit where the set of arms in round $t$ is $\mathcal{A}_t \subseteq \mathbb{R}^d$. The arm is $a \in \mathcal{A}_t$ and its mean reward is $a^\top \theta_*$. Explain that this model is as general as it gets, since changing $\mathcal{A}_t$ can be used to model context.

* Define cumulative regret. No talking about constraints or explainability yet.

\textbf{Section 4: Explainable Exploration with Side Constraints}
\todoz{I would prefer to starting with the unconstrained ones as we won't have analysis for it anyway. Then, in the extension, we present the constraints, and demonstrate our approach can easily incorporate side constraints. We could leave it in the motivation though.}
* Introduce the algorithm in the linear bandit setting. Two types of constraints:

o Side constraints of the form $M_t \pi_t \geq b_t$.

o Eliminated arms in $\mathcal{A}_t$, their UCB is lower than the highest LCB, are not included.

o Have $\sqrt{\log(1 / \delta)}$ in confidence intervals, where $\delta > 0$ is the failure probability. In experiments, we can choose $\delta = 0.05$ and be comparable to TS.

* Discuss key properties of the algorithm design:

o Interpretability by design.

o Linear side constraints by design. This is a plenty for promotions and fairness. Give examples.

o The constraints can also represent acceptable production policies. We solve an optimization problem to explore optimally within these constraints.

o Optimal designs are a common design principle. Our contribution here is that we drop phases. Theoreticians will love it. Quadrupling phases are a horrible idea when the set of arms changes.

\smnote{Real problems always needs explainabality}

\textbf{Section 5: Multi-Armed Bandit Analysis}
\todoz{I would also suggest that we put this as a subsection of the previous section. This serves as a warm up.}
* This is a warm-up section. We do not analyze side constraints. We need to have a good excuse for this. One possibility is that the constraints can be quite arbitrary.

* Rewrite the algorithm for MAB. The algorithm pulls the least-pulled non-eliminated arms with the same probability.

* The same bound as other MAB methods.

* Key ideas in the analysis. This is mostly standard.

\textbf{Section 6: Linear Bandit Analysis}

* This is the main technical section. We do not analyze side constraints. We need to have a good excuse for this. One possibility is that the constraints can be quite arbitrary.

* The same bound as other linear bandit methods.

* The main trick, the one-step look-ahead norm, should be a lemma. Roughly speaking, it is
\begin{align*}
  \langle A_t^*,\theta_*\rangle- \sum_{a\in\cA_t}\pi_t(a)\langle a,\theta_*\rangle
  \leq \left(2+S\right)\sum_{a\in\cA_t}\pi_t(a)\|a\|_{V_t^{-1}}\sqrt{\beta_t+LS}\,.
\end{align*}

* If space permits, present the proof of the above.

\textbf{Section 7: Experiments}

* Comparison to LinTS, LinUCB, and phase-based arm elimination. No side constraints. We are not much worse than LinTS and LinUCB, and much better than phase-based designs.

* Changing side constraints. Compare to LinTS that naively satisfies the side constraints. This can be implemented as follows:

o Compute an empirical distribution of TS over pulled arms.

o Project to the closest vertex of the simplex of policies that satisfy the side constraints. This can be solved as LP when the similarity is a dot product.

\textbf{Section 8: Conclusions}

{\color{red} End of paper outline}

The non-phased optimal design algorithm can be something like in \Cref{alg:linear-bandit}.
\begin{algorithm}[!tbh]
\caption{G-optimal Design with Elim}
% \label{alg:linear-bandit}
\begin{algorithmic}[1]
\State Input: Finite set $\X \subset \mathbb{R}^d$.
\State Let $\X_1 \leftarrow \X, \ell \leftarrow 1$
\While{$\ell = 1,2,\ldots, T$}
\State Let $\widehat{\lambda}_{\ell} \in \Delta_{\X_{\ell}}$ be a $\frac{d(d+1)}{2}$-sparse minimizer of 
$$
f(\lambda)=\max _{\bx \in \X_{\ell}}\|\bx\|_{\left(\sum_{\bx \in \X_{\ell}} \lambda_{\bx} \bx \bx^{\top}\right)^{-1}}^2 \quad \text{/*G-optimal design*/}
$$\todoz{I think we need D-optimal here. The equivalency between G and D might not hold. But this is minor as both of them are explainable.}
\State Sample arm $\bx\in\X_{\ell}\sim \widehat{\lambda}_{\ell}$
% \State Set $\epsilon_{\ell}=2^{-\ell}, \tau_{\ell}=2 d \epsilon_{\ell}^{-2} \log \left(4 \ell^2|\X| / \delta\right)$
% \State Pull arm $\bx \in \X$ exactly $\left\lceil\widehat{\lambda}_{\ell, \bx} T_{\ell}\right\rceil$ times 
and construct the least squares estimator $\wtheta_{\ell}$
\State Set $\epsilon_\ell = 1/\sqrt{\ell}$. Eliminate arms such that
\begin{align*}
& \X_{\ell+1} \leftarrow \X_{\ell} \backslash\left\{\bx \in \X_{\ell}: \max_{\bx^{\prime} \in \X_{\ell}}\left\langle \bx^{\prime}-\bx, \wtheta_{\ell}\right\rangle>2 \epsilon_{\ell}\right\} \quad \text{/*UCB-LCB comparison*/}
\end{align*}
\If{$\left|\X_{\ell}\right|=1$}
\State Sample the arm till $T$
\EndIf
\State $\ell \leftarrow \ell+1$
\EndWhile
\end{algorithmic}
\end{algorithm}

Note that due to Kiefer-Wolfowitz's statement, we have that G-optimal design is equivalent to D-optimal design. So we can replace line 4 as follows:
\begin{align*}
    \widehat{\lambda}_\ell = \max_\lambda \log \left(\left|\sum_{\bx \in \X_{\ell}} \lambda_{\bx} \bx \bx^{\top}\right|\right)
\end{align*}




Notations: Let $\mathcal{A}=[K]:=\{1, \ldots, K\}$ be a tabular action set. When action $a \in \mathcal{A}$ is taken, we observe its stochastic reward with (initially) unknown mean $\bar{r}(a) \in[0,1]$. A policy $\pi: \mathcal{A} \rightarrow[0,1]$ is a probability distribution on $\mathcal{A}$ and we denote by $\Pi$ the set of all possible policies. Following Section 21.1 of Lattimore and Szepesvári [2020], we use the terms "policy" and "design" interchangeably. To simplify notation, we use $\bar{r}$ and $\pi$ to denote the vectorized expected reward and the policy, i.e., $\bar{r}=(\bar{r}(1), \ldots, \bar{r}(K)) \mathbf{T}$ and $\pi=(\pi(1), \ldots, \pi(K)) \mathbf{T}$. The expected reward of policy $\pi$ is thus $V(\pi ; \bar{r})=\pi^{\top} \bar{r}$ (when the context is clear enough, we may also suppress the explicit dependence on $\bar{r}$. For any $p \geq 0$, we define $\|\cdot\|_p$ as the $p$-norm and $\Delta_{A-1}=\left\{x \in \mathbb{R}^k: x \geq 0,\|x\|_1=1\right\}$ as the $k$-dimensional simplex. For any $c \in \mathbb{R}$, we use $c \mathbf{1}_k$ to denote the $k$-dimensional vector with all entries equal to $c$ (when $c=0$, we write this as $\mathbf{0}_k$ ). We use $\mathbb{1}\{\cdot\}$ to denote the indicator function. For two vectors $a, b$ with same dimension, we use $a \circ b$ to denote their Hadamard (coordinate-wise) product. A random variable $X$ is $\sigma^2$-sub-Gaussian if $\mathbb{E}[X]=0$ and its moment generating function satisfies $\mathbb{E}[\exp (s X)] \leq \exp \left(s^2 \sigma^2 / 2\right)$ for all $s \in \mathbb{R}$.

Setting: Let $\mathcal{A}=\left\{a_1, \ldots, a_n\right\} \subseteq \Re^d$ be a fixed action set and $K=|\mathcal{A}|$ be the cardinality of $\mathcal{A}$. Choosing action $A_t$ at time step $t$ would generate a reward $X_t=\left\langle\theta_*, A_t\right\rangle+\eta_t$, where $\eta_t$ is conditionally 1-sub-Gaussian. We use $\pi_t$ to denote a distribution over $\mathcal{A}$ of time $t$ and $V_t=$ $\sum_{s=1}^{t-1} A_s A_s^{\top}$ be the design matrix up to time $t$.
At time $t$, we sample an action $A_t$ according to $\pi_t$. $\pi_t$ is computed via the following optimization program:
$$
\begin{array}{ll}
\max _\pi & \log \operatorname{det}\left(V_t+\sum_{a \in \mathcal{A}_t} \pi(a) a a^{\top}\right) \\
\text { s.t. } \pi \in \Delta_{\left|\mathcal{A}_t\right|-1} \\
& \left(\max _{\theta \in \mathcal{C}_t}\langle a, \theta\rangle-\min _{\theta \in \mathcal{C}_t}\left\langle a^{\prime}, \theta\right\rangle\right) \pi(a) \geq 0 \quad \forall a, a^{\prime} \in \mathcal{A}_t .
\end{array}
$$
Here, $\mathcal{C}_t$ is the confidence region for $\theta_*$ up to time step $t$.

\subsection{Linear Bandit proof outline}

\noindent\textbf{Method 1:} If we just solve \eqref{eq:d_optimal} greedily to acquire a single action $A_t$ for time step $t$ (\ie, we restrict that $\pi_t$ would deterministically select an action that maximizes the objective in \eqref{eq:d_optimal}), then it is definitely true that one can upper bound the confidence interval for any action $a$ as follows
\begin{align}\label{eq:logdet1}
1\wedge\|a\|^2_{V^{-1}_t}\leq\log\det(V_t+aa^{\top})-\log\det(V_t)\leq\log\det(V_t+A_tA^{\top}_t)-\log\det(V_t),
\end{align}
where the second inequality holds by definition of $A_t$ and $\pi_t.$ This shall give us the desire upper bound if we apply this with $a$ being $A^*_t$ and $A_t$, respectively.

\noindent\textbf{Method 2:} However, as we know, the optimal $\pi_t$ for \eqref{eq:d_optimal} is likely to be a distribution over $\cA_t.$ Now if we re-apply \eqref{eq:logdet1}, we would have 
for any action $a,$ it holds
\begin{align}\label{eq:logdet2}
1\wedge\|a\|^2_{V^{-1}_t}\leq\log\det(V_t+aa^{\top})-\log\det(V_t)\leq\log\det\left(V_t+\sum_{b'\in\cA_t}\pi_t(b)bb^{\top}\right)-\log\det(V_t).
\end{align}
\smnote{it should be just $b$}

where the second inequality holds again by definition of $\pi_t.$ Note that $\pi_t$ now is a distribution over $\cA_t$ and the log determinant function is concave (so we cannot apply Jensen's inequality to the last step to get an upper bound). It becomes challenging to apply the log determinant inequality from this step on.

One way to bypass this is to consider another norm in the analysis. Recall that, at time $t$, we sample an action $A_t$ according to $\pi_t.$ $\pi_t$ is computed via the following optimization program:
\begin{align}
  \max_\pi \ &\log\det\left(V_t+\sum_{a\in\cA_t}\pi(a)aa^{\top}\right)  \label{eq:d_optimal_duplicate}\\
  %%%%%%%%%%%%%%%%%%%%
  \mathrm{s.t.} \
  & \pi\in\Delta_{|\cA_t|-1} \nonumber \\ 
  %%%%%%%%%%%%%%%%%%%%
  & \left(\max_{\theta\in\cC_t}\langle a,\theta\rangle-\min_{\theta\in\cC_t}\langle a',\theta\rangle\right)\pi(a)\geq 0\quad\forall a,a'\in\cA_t\,.\nonumber
\end{align}
Here, $\cC_t$ is the confidence region for $\theta_*$ up to time step $t$. We can easily find that the expected regret of time step $t$ is 
\begin{align}
    &\nonumber\langle A_t^*,\theta_*\rangle- \sum_{a\in\cA_t}\pi_t(a)\langle a,\theta_*\rangle\\
    %%%%%%%%%%%%%%%%%%%%%%%%%
    =&\nonumber\langle A_t^*,\theta_*\rangle-\min_{\theta\in\cC_t}\langle A^*_t,\theta\rangle+\min_{\theta\in\cC_t}\langle A_t^*,\theta\rangle-\sum_{a\in\cA_t}\pi_t(a)\left(\max_{\theta\in\cC_t}\langle a,\theta\rangle-\max_{\theta\in\cC_t}\langle a,\theta\rangle+\langle a,\theta_*\rangle\right)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    =&\nonumber\langle A_t^*,\theta_*\rangle-\min_{\theta\in\cC_t}\langle A^*_t,\theta\rangle + \underbrace{\min_{\theta\in\cC_t}\langle A_t^*,\theta\rangle-\sum_{a\in\cA_t}\pi_t(a)\max_{\theta\in\cC_t}\langle a,\theta\rangle}_{\textbf{\smnote{Constraint, assume $\pi_t$ is deterministic}}}-\sum_{a\in\cA_t}\pi_t(a)\left(-\max_{\theta\in\cC_t}\langle a,\theta\rangle+\langle a,\theta_*\rangle\right)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    \leq&\langle A_t^*,\theta_*\rangle-\min_{\theta\in\cC_t}\langle A_t^*,\theta\rangle-\sum_{a\in\cA_t}\pi_t(a)\left(-\max_{\theta\in\cC_t}\langle a,\theta\rangle+\langle a,\theta_*\rangle\right)\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    =&\langle A_t^*,\theta_*\rangle-\min_{\theta\in\cC_t}\langle A_t^*,\theta\rangle+\sum_{a\in\cA_t}\pi_t(a)\left(\max_{\theta\in\cC_t}\langle a,\theta\rangle-\langle a,\theta_*\rangle\right).\label{eq:ci}
\end{align}
Here, the inequality is due to the second constraint of \eqref{eq:d_optimal_duplicate}. The second term of \eqref{eq:ci} can be upper-bounded as 
\begin{align}
    \sum_{a\in\cA_t}2\pi_t(a)\|a\|_{V_t^{-1}}\sqrt{\beta_t},
\end{align}
where $\beta_t$ is the width of $\cC_t$, the confidence region of $\theta$.


For the first term of \eqref{eq:ci}, we leverage the first order optimality criterion to derive a ``one-step lookahead" norm inequality. Denoting $\theta_{t,a}=\argmin_{\theta\in\cC_t}\langle a,\theta\rangle,$ the confidence interval for any $a$ could also be upper bounded by Cauchy-Schwarz inequality as
\begin{align}
    |\langle a,\theta_*-{\theta}_{t,a}\rangle|\leq&\|a\|_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}\|\theta_*-\theta_{t,a}\|_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})}\\
\leq&\|a\|_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}\sqrt{\beta_t+LS},\label{eq:ci2}
\end{align} \todob{Can you comment on how this arises? I assume that $\beta_t$ is from concentration and $L S$ is a trivial upper bound on the rest.}
\todoz{Yes, you are absolutely right. It's $\|\theta_*-\theta_{t,a}\|_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})}=\|\theta_*-\theta_{t,a}\|_{V_t}+\|\theta_*-\theta_{t,a}\|_{\sum_{a\in\cA_t}\pi_t(a)aa^{\top}}\leq\sqrt{\beta_t}+\sqrt{LS}$, where the last step follows from Cauchy-Schwarz.}
\smnote{in (17) are you missing an inverse. Should it be $\|\theta_*-\theta_{t,a}\|_{(V_t + \sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}$.Next, can you give me a reference of this identity: $\|\theta_*-\theta_{t,a}\|_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}=\|\theta_*-\theta_{t,a}\|_{V_t^{-1}}+\|\theta_*-\theta_{t,a}\|_{(\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}$. Searched around a bit but could not find it. Or what you are doing in (17) is like a crude upper bound. Observe that $\|\theta_*-\theta_{t,a}\|_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}\leq \|\theta_*-\theta_{t,a}\|_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})}$. This could be loose, but the scaling of $\sqrt{T}$ is probably fine.}

where $L\geq \|\theta_*\|$ and $S\geq\|a\|$ are the $\ell_2$-norm upper bound of the parameter and the arm vectors. For the first term of \eqref{eq:ci2}, by the first order optimality condition of D-optimal design, we have for any arm $a$, and in particular, the optimal arm $A_t^*$,
\begin{align}  \|A_t^*\|^2_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}\leq&\sum_{a\in\cA_t}\pi_t(a)\|a\|^2_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}\\
\leq&\sum_{a\in\cA_t}\pi_t(a)\|a\|^2_{V_t^{-1}}\leq S\sum_{a\in\cA_t}\pi_t(a)\|a\|_{V_t^{-1}},
\end{align} \todob{Can you comment on the first order optimality condition of D-optimal design? How does $\log\det$ maximization imply the first inequality? This is the most interesting part of the proof.} 
\todoz{This uses the tools outlined in Theorem 21.1 of Chapter 21.1 in \cite{lattimore2020bandit}. For the optimal solution of optimal design, we have for any $\pi$, it holds (due to the first order optimality condition) $\sum_{a\in\cA_t}\pi(a)\|a\|^2_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}\leq\sum_{a\in\cA_t}\pi_t(a)\|a\|^2_{(V_t+\sum_{a\in\cA_t}\pi_t(a)aa^{\top})^{-1}}$. Setting $\pi$ to be atomic on $A_t^*$ gives the desired inwquality.}

\todob{I thought that the argument can be simplified as

$\|A_t^*\|^2_{V_t^{-1}}$

$\lesssim \log\det(V_t + A_t^* (A_t^*)^\top) - \log\det(V_t)$

$\leq \log\det(V_t + \sum_{a\in\cA_t}\pi_t(a)aa^\top) - \log\det(V_t)$

$\leq \sum_{a\in\cA_t} \pi_t(a) \log\det(V_t + aa^\top) - \log\det(V_t)$

The first inequality is standard, the second is from D optimality, and the last is from the concavity of $\log\det$. There is an issue in the last step though. I assume that this is what you faced initially.}

\todoz{You are totally correct! This only works if $\pi_t$ is atomic, which is the case for one-step greedy approximation.}
where we have assumed that $V_1= I.$

Combining the above and put them back to \eqref{eq:ci}, we have the expected regret of a time step $t$ is at most 
\begin{align}
    \left(2+S\right)\sum_{a\in\cA_t}\pi_t(a)\|a\|_{V_t^{-1}}\sqrt{\beta_t+LS},
\end{align}
Sum of this over $t=1,\ldots,T$ is roughly $O(\sqrt{T})$ away from $$\left(2+S\right)\sum_{t=1}^T\|A_t\|_{V_t^{-1}}\sqrt{\beta_t+LS}.$$
From here, we can apply the usual log determinant inequality.

\smnote{We may also have to talk about the rounding procedure we have to do at every round. See Appendix B of \citet{fiez2019sequential}}

{\color{blue} RZ: why do we need rounding here?}

\todob{I do not think that rounding will be needed. The bound will be proved in expectation over the randomness in sampled actions.}
\todoz{I agree with what Brano said above, the algorithm would just sample according to $\pi_t$ and regret shall be proved in expectation.}
%\noindent\textbf{Summary:} In short, both methods shall give us the desire $O(d\sqrt{T})$ regret upper bound. But I suspect that the second approach would be more convenient when we go to the scenario with more constraints.


\smnote{I went over the proof. Somehow, I cannot see how the elimination constraints are taking effect. Don't we need something like this. I think when we are going from (14) to (15) we require this}

Define the good event that the optimal arm $A^*_t$ survives and eliminates the sub-optimal arm $a$
\begin{align*}
    \xi_{elim, t} \coloneqq \{\min t: \max_{\theta\in\cC_t}\langle A^*_t,\theta\rangle-\min_{\theta_\in\cC_t}\langle a,\theta\rangle \geq \sqrt{\beta_t(\delta)}\}
\end{align*}

Also, I guess we will directly use Theorem 2 from \citet{abbasi2011improved} to bound the confidence width
$$
C_t^{}=\left\{\theta \in \mathbb{R}^d:\left\|\widehat{\theta}_t-\theta\right\|_{\bar{V}_t} \leq \underbrace{R \sqrt{d \log \left(\frac{1+t L^2 / \lambda}{\delta}\right)}+\lambda^{1 / 2} S}_{\beta_t(\delta)}\right\}
$$

==> lin_bandit_opt_app.tex <==
As one can see in the proof of \cref{thm:lin-bandit} that, when $K$ (the cardinality of the action set in each round) grows large, the regret of \code may become sub-optimal by a factor of $\sqrt{d}$. Comparing the K-armed bandits and the linear bandits, we can conclude that part of this can be attributed to the randomness in $\pi_t$, which brings additional challenges in the analysis (see, \emph{e.g.}, \cref{lemma:one-step} and \cref{lemma:conc-sampling}).

In this section, we present an greedy approximation of \code, which removes the randomness in $\pi_t$ to avoid the above-mentioning issue. Specifically, in each round $t$, \code selects an action according to $\pi_t$, which is computed as follows:
\begin{align}
\pi_t = &\argmax_\pi  \log \operatorname{det}\left(V_t+\sum_{a \in \A_t} \pi(a) a a^{\top}\right) \nonumber\\
 &\text { s.t. } \pi \in \Delta_{\left|\A_t\right|-1} \nonumber\\
& \pi(a)\left(\max _{\btheta \in \mathcal{C}_t}\langle a, \btheta\rangle-\min _{\btheta \in \mathcal{C}_t}\left\langle a^{\prime}, \btheta\right\rangle\right)  \geq 0 \quad \forall a, a^{\prime} \in \A_t\,\nonumber\\
& \sum_{a\in\cA_t}\pi^2(a)=1.
\label{eq:d_optimal_greedy}
\end{align}
The only difference between \eqref{eq:d_optimal_greedy} and \eqref{eq:d_optimal} is the additional inclusion of the last constraint, which demands that $\pi_t$ should put all weights to one single action. This is because
\begin{align*}
\sum_{a\in\cA_t}\pi^2(a)\leq \sum_{a\in\cA_t}\pi(a)=1,
\end{align*}
and equality holds only when one of the $\pi(a)$'s is 1 and all others are 0.

Suppose we instantiate $V_t$ and $\cC_t$ the same as \cref{sec:lin-bandit}, we would have from \cref{lemma:per-step-regret} that, under the good event $\xi_n$, the expected regret in round $t$ is at most
\begin{align}\label{eq:greedy_code_regret1}
        \langle A_t^*,\btheta_*\rangle- \sum_{a\in\cA_t}\pi_t(a)\langle a,\btheta_*\rangle\leq\langle A_t^*,\btheta_*\rangle-\min_{\btheta\in\cC_t}\langle A_t^*,\btheta\rangle+\left(\max_{\btheta\in\cC_t}\langle A_t,\btheta\rangle-\langle A_t,\btheta_*\rangle\right),
\end{align}
where we recall $A_t$ is now the action deterministically selected by $\pi_t$. Following existing works in linear bandits (see, \emph{e.g.}, \cite{abbasi2011improved}), the second term in \eqref{eq:greedy_code_regret1} can be upper bounded as $\min\{1,\|A_t\|_{V^{-1}_t}\|\}2\sqrt{\beta_t(\delta)}$ (notice that the expected regret in each round is at most 1). Summing this from $t=1,\ldots,n$ one can apply the log-determinant inequality (\cref{lemma:supp-1}) to show that this is at most $\tilde{O}(d\sqrt{n})$. 

For the first term in \eqref{eq:greedy_code_regret1}, note that the per round expected regret is at most 1, applying the Cauchy-Schwarz inequality, we have
\begin{align*}
\min\left\{1,\langle A_t^*,\btheta_*\rangle-\min_{\btheta\in\cC_t}\langle A_t^*,\btheta\rangle\right\}\leq&\min\left\{1, \|A^*_t\|_{V^{-1}_t}\max_{\btheta\in\cC_t}\|\btheta-\btheta_*\|\right\}\\
\leq&2\sqrt{\beta_t(\delta)}\min\{1,\|A^*_t\|_{V^{-1}_t}\}\leq2\sqrt{\beta_n(\delta)}\min\{1,\|A^*_t\|_{V^{-1}_t}\},
\end{align*}
where we have made use of $\beta_n(\delta)\geq\beta_t(\delta)\geq 1$. Summing the above over from $t=1,\ldots,n$ we have
\begin{align}
\nonumber\sum_{t\in[n]}\min\left\{1,\langle A_t^*,\btheta_*\rangle-\min_{\btheta\in\cC_t}\langle A_t^*,\btheta\rangle\right\}\leq&2\sqrt{\beta_n(\delta)}\sum_{t\in[n]}\min\{1,\|A^*_t\|_{V^{-1}_t}\}\\
\leq&2\sqrt{n\beta_n(\delta)\sum_{t\in[n]}\min\{1,\|A^*_t\|^2_{V^{-1}_t}\}}\label{eq:greedy_code_regret2}\\
\leq&2\sqrt{n\beta_n(\delta)\sum_{t\in[n]}\log\left(1+\|A^*_t\|^2_{V^{-1}_t}\right)}\label{eq:greedy_code_regret3},
\end{align}
where \eqref{eq:greedy_code_regret2} follows from the Cauchy-Schwarz inequality and \eqref{eq:greedy_code_regret3} follows from the fact that $y\leq 2\log(1+y)$ for all $y\in[0,1]$.

Now from the proof of Lemma 19.4 in \cite{lattimore2020bandit}, we have for any $a\in\cA_t$,
\begin{align*}
\log\left(1+\|a\|^2_{V^{-1}_t}\right)=\log\det(V_{t}+aa^{\top})-\log\det(V_{t}).
\end{align*}
Since $A_t$ is chosen such that $\log\det(V_{t}+A_tA_t^{\top})$ is maximized among all $a\in\cA_t$, we have 
\begin{align}
\nonumber\log\left(1+\|A^*_t\|^2_{V^{-1}_t}\right)=&\log\det(V_{t}+A^*_t(A^*_t)^{\top})-\log\det(V_{t})\\
\leq&\log\det(V_{t}+A_tA_t^{\top})-\log\det(V_{t})=\log\left(1+\|A_t\|^2_{V^{-1}_t}\right).\label{eq:greedy_code_regret4}
\end{align}
Putting \eqref{eq:greedy_code_regret4} back into \eqref{eq:greedy_code_regret3} for $t=1,\ldots,n$, we have
\begin{align}
\nonumber\sum_{t\in[n]}\min\left\{1,\langle A_t^*,\btheta_*\rangle-\min_{\btheta\in\cC_t}\langle A_t^*,\btheta\rangle\right\}\leq&2\sqrt{n\beta_n(\delta)\sum_{t\in[n]}\log\left(1+\|A_t\|^2_{V^{-1}_t}\right)}.
\end{align}
One can thus apply the log-determinant inequality in \cref{lemma:supp-1} to upper bound this term as $\tilde{O}(d\sqrt{n})$ as well.

==> reward_free.tex <==
\section{Reward Free RL}
\textbf{Brano's question:} How are optimal designs different from more active approaches, such as taking the action with the highest uncertainty (as above)? The latter is obviously a heuristic for variance minimization. But how bad can it be? I am pretty sure that the old folks would not invent optimal designs and wrote them down as optimization problems if there were simple greedy solutions.

\textbf{Answer:} Yes, solving those optimization problems is not easy. To understand this, first, let us look into \citet{jin2020reward}. This is a tabular RL setting where during the exploration phase you do not have access to the reward function. Once the exploration data is collected, then you get access to the reward function. The RL objective is to find an $\epsilon$-optimal policy $\pi$, satisfying
\begin{align*}
\mathbb{E}_{s_1 \sim \mathbb{P}_1}\left[V_1^{\star}\left(s_1\right)-V_1^\pi\left(s_1\right)\right] \leq \epsilon
\end{align*}
where, $V_1^\pi\left(s_1\right)$ is estimated from the collected dataset. In theorem 3.5 they show that they require $H^5 S^2 A \imath / \epsilon^2$ samples for a $\epsilon$-optimal policy.

\begin{customtheorem}{3.5}
There exists absolute constant $c>0$, for any $\epsilon>0, p \in(0,1)$, assume dataset $\mathcal{D}$ has $N$ i.i.d. samples from distribution $\mu$ which satisfies Eq. (4) with $\delta=\epsilon /\left(2 S H^2\right)$, and $N \geq c H^5 S^2 A \imath / \epsilon^2$, then with probability at least $1-p$, for any reward function $r$ simultanouesly, the output policy $\hat{\pi}$ of Algorithm 3
\begin{align*}
\mathbb{E}_{s_1 \sim \mathbb{P}_1}\left[V_1^{\star}\left(s_1 ; r\right)-V_1^{\hat{\pi}}\left(s_1 ; r\right)\right] \leq 3 \epsilon
\end{align*}
\end{customtheorem}
The key idea in this paper is to distinguish between significant and insignificant states. The significant states are those state that can be reached with high probability starting from the starting state (see definition 3.2). The key idea is to upper bound the visitation to the significant states which yields the above theorem result.

I think given no context and structure this is the best or near best you can do. They also have a lower bound which shows that $\Omega\left(S^2 A H^2 / \epsilon^2\right)$ trajectories must be collected to yield $\epsilon$-optimal policy.


For the linear RL setting, we can look into this paper \citet{wagenmaker2022reward}. They consider the linear RL setting as proposed in \citet{jin2020provably}. Further, they propose an algorithm that does $G$-optimal design to cover all trajectories. However, solving this optimal design problem is difficult in the RL setting. So they crucially design the regret minimization algorithm with a special reward as follows:
\begin{align*}
    r(\phi ; \Lambda) \leftarrow\left\{\begin{array}{cc}
1 & \|\phi\|_{\Lambda^{-1}}^2>\gamma^2, \phi \in \mathcal{X} \\
\frac{1}{\gamma^2}\|\phi\|_{\Lambda^{-1}}^2 & \|\phi\|_{\Lambda^{-1}}^2 \leq \gamma^2, \phi \in \mathcal{X} \\
0 & \phi \notin \mathcal{X}
\end{array}\right.
\end{align*}
then it yields a solution close to the solving the G-optimal design problem in RL. This is computationally less intensive then solving the G-optimal design problem. This Cover Traj algorithm is shown in Algorithm 4. Finally once this data us collected then we can use Algorithm 2 in the planning phase to get the following theorem 
\begin{customtheorem}{1}
Consider running RFLIN-EXPLORE with tolerance $\epsilon>0$ and confidence $\delta>0$, and let RFLIN-PLAN $(\cdot)$ denote its output. Then with probability at least $1-\delta$, for an arbitrary number of reward functions $r$ satisfying Definition 3.1, RFLIN-PLAN $(r)$ returns a policy $\widehat{\pi}$ which is $\epsilon$-optimal with respect to $r$. Furthermore, this procedure collects at most
\begin{align*}
\widetilde{\mathcal{O}}\left(\frac{d H^5(d+\log 1 / \delta)}{\epsilon^2}+\frac{d^{9 / 2} H^6 \log ^4(1 / \delta)}{\epsilon}\right)
\end{align*}
episodes, where $\widetilde{\mathcal{O}}(\cdot)$ hides absolute constants and terms poly $\log (d, H, 1 / \epsilon)$ and poly $\log \log (1 / \delta)$.
\end{customtheorem}

For $\epsilon$ sufficiently small, exploring via RFLIN-EXPLORE and planning via RFLIN-PLAN learns an $\epsilon$-optimal policy for an arbitrarily large number of reward functions using only $\mathcal{O}\left(\frac{d^2 H^5}{\epsilon^2}\right)$ episodes. This improves on both existing reward-free algorithms for linear MDPs by a factor of $d$ (Zanette et al., 2020c; Wang et al., 2020).

Remark 4.1 (Computational Efficiency). In MDPs with a finite number of actions, both RFLIN-EXPLORE and RFLINPLAN are computationally efficient, with computational cost scaling polynomially in $d, H, 1 / \epsilon, \log 1 / \delta$, and $|\mathcal{A}|$. The primary computational cost of RFLIN-EXPLORE is due to COVERTRAJ, while the computational cost of RFLINPLAN is due primarily to solving a least-squares problem.


Theorem 1 shows that we can learn $\epsilon$-optimal policies for all valid reward functions simultaneously, without having access to the reward functions during exploration, using only $\widetilde{\mathcal{O}}\left(d^2 H^5 / \epsilon^2\right)$ episodes. In other words, up to $H$ factors, reward-free RL is no harder than reward-aware $R L$ in linear MDPs. This is in contrast to the tabular setting, where it is well known that the optimal rate for reward-aware $\mathrm{RL}$ is $\Theta\left(|\mathcal{S} \| \mathcal{A}| / \epsilon^2\right)$ while the optimal rate for reward-free $\mathrm{RL}$ is $\Theta\left(|\mathcal{S}|^2|\mathcal{A}| / \epsilon^2\right)$.


\smnote{So in short you don't need to solve the G-optimal design problem in linear RL. You can approximate its solution using the RegMin (low regret) algorithm with a special reward function.}

\textbf{Future Directions:} I think it is interesting to consider two directions:
\begin{enumerate}
    \item Weakly revealing reward function: I think having no access to reward function during exploration phase is a very strong assumption. What happens when you only can access the reward function a fixed budget of $B$ times (small) during the exploration phase. How much speedup do you get?
    \item What happens when you have access to the offline data $\D$ which includes data like $\{s_t,a_t,r_t,s'_t\}_{t=1}^H$ for a few episodes. How much speedup in learning do you get?
    \item Is there a connection between this and data collection for policy evaluation under reward-free setting?
\end{enumerate}

